How to Retrain Recommender System? A Sequential Meta-Learning Method

Practical recommender systems need be periodically retrained to refresh the model with new interaction data. To pursue high model fidelity, it is usually desirable to retrain the model on both historical and new data, since it can account for both long-term and short-term user preference. However, a full model retraining could be very time-consuming and memory-costly, especially when the scale of historical data is large. In this work, we study the model retraining mechanism for recommender systems, a topic of high practical values but has been relatively little explored in the research community. Our first belief is that retraining the model on historical data is unnecessary, since the model has been trained on it before. Nevertheless, normal training on new data only may easily cause overfitting and forgetting issues, since the new data is of a smaller scale and contains fewer information on long-term user preference. To address this dilemma, we propose a new training method, aiming to abandon the historical data during retraining through learning to transfer the past training experience. Specifically, we design a neural network-based transfer component, which transforms the old model to a new model that is tailored for future recommendations. To learn the transfer component well, we optimize the "future performance" -- i.e., the recommendation accuracy evaluated in the next time period. Our Sequential Meta-Learning(SML) method offers a general training paradigm that is applicable to any differentiable model. We demonstrate SML on matrix factorization and conduct experiments on two real-world datasets. Empirical results show that SML not only achieves significant speed-up, but also outperforms the full model retraining in recommendation accuracy, validating the effectiveness of our proposals. We release our codes at: https://github.com/zyang1580/SML.

==> 5_experiments.tex <==
\section{EXPERIMENTS}\label{sec:experiment}
\quad In this section, we present our experimental setup on two dataset with different properties.
We design experiments to answer the following questions:\\
\begin{itemize}
    \item[\textbf{RQ1:}] Does our method achieve better performance compared with state-of-the-art sequential recommendation models?
    \item[\textbf{RQ2:}] How the various components in Transfer model influence the performance?
    \item[\textbf{RQ3:}] What is the influence of various hyper-parameters of CNN framework?
\end{itemize}

\subsection{Experiments Setting}
A. Datasets\\
\quad We evaluate our methods on two real world datasets. In order to simulate the real world data flow, we divide the data set into several parts in chronological order. For dataset D, we divide it into \{D$_0$,D$_1$.....,D$_n$\}. In training period t, we will train our transfer model only on D$_t$, and then test on D$_{t+1}$. When test is over, we go to the next period of training. For new items and users in current test period, we initialized their embedding by the same Gaussian distribution. The statistics of the datasets are shown in Table1.\\
Yelp2019\\
The dataset is from Yelp Dataset Challenge round 13, which contains more than 6 million user reviews . The time span is nearly 10 years. It can well reflect the long-term interests evolution of users. During data cleansing, we remove the interactions from extremely inactive users whose total interaction less than 10.\\
Adressa\\
The Adressa Dataset is a news dataset that includes news articles in connection with anonymized users. It recorded 3,664,225 clicks by 478,612 people in three weeks. Thererfore, the dataset is highly sparse and time sensitive.\\

For the Yelp dataset, we sort the interactions by time and divide them into 40 parts according to the number of interactions. In our settings, 10 of them are used for pre-training, 20 for phased training, 3 for evaluation, and 7 for test. As for Adressa dataset, we divide it into 63 parts according to the time span, 21 for pre-training , 24 for phased training, 5 for evaluation, and 10 for test. We take the weighted average result as the final result. When testing, we perform random negative sampling from the items that have appeared, and the negative sampling of the Adressa dataset is only performed on the items that have appeared in the last 3 periods, because news is time sensitive.\\

B.Baselines\\
We compare our methods with three variants of Matrix Factorization,two state-of-the-art sequential recommendation models and a streaming recommendation method. \\

Full Training MF: We full retrain the MF model based on \{D$_0$,D$_1$.....,D$_n$\} and test performance on $D_{t+1}$. Hyper-parameters are fixed before first period training.

Fine Tuning MF: Based on MF model, use only Dt as training set when test on Dt+1. Furthermore, we train on the basis of the parameters trained in the previous period.\\

GRU4Rec:A RNNs based method that uses user interaction sequence for session-based recommendation. We treat all of one’s interaction in D1....Dt as a session.This model has poor performance under the experimental settings of the original article. For fair comparison, we change the negative sampling during GRU4Rec training to negative sampling in all the items that have appeared. \\

Convolutional Sequence Embeddings(Caser):A powerful CNN-based model capturing evolution in interest by convolution calculations on the picture constructed of historical interaction. We make the target items of caser training sequence in Dt, and tuning length of the sequence to achieve best performance. Items outside the target in the sequence may not appear in Dt. other settings inherit settings from the article.\\

SRMF:Streaming Ranking Based Recommender System is a latest online method. It develops a reservoir to represent user historical interest by statistical  and update the reservoir over time.\\

For fair comparison, all the methods use Adam optimizer. We consider the latent dimension from \{32,64,128,256\}, the l2 regularizer is from \{0.01,0.001,0.0001,0.00001,0.000001\}, and the learning rate lr is from \{0.01,0.001,0.0001\}. We make adjustments every 10 epochs until each method achieves its best performance on evaluation set.\\
C.Pre-training\\
For all the baselines, we train them on \{D1...Dk\} until achieving the best performance on $D_(k+1)$. k is equal to 47 for Adressa, and 29 for Yelp. For our method, we  pre-train MF base model's parameter and randomly initialize the Transfer model's parameter. At this point,k is equal to 20 for Adressa, and 9 for Yelp.






\begin{table*}
  \caption{result of news}
  \label{tab:news-result}
  \begin{tabular}{ccccccl}
    \toprule
    methods &Recall@5 & Recall@10&Recall@20 & NDCG@5&NDCG@10&NDCG@20\\
    \midrule
    MF-full-retraining & 0.04692& 0.0883& 0.1601 & 0.0285 & 0.0417 &0.0597 \\
    MF-fine-tuning & 0.1086& 0.2280 & 0.3775 & 0.0606&0.0989& 0.1367\\
    SPMF\_(7k-15w pool) &0.1060& 0.2134& 0.3611& 0.0560& 0.0943& 0.1316 \\
 %   SPMF\_(7k-15w pool base1e-2) &0.1060& 0.2134& 0.3611& 0.0560& 0.0943& 0.1316 \\
    GRU4Rec & 0.0163& 0.0329& 0.0680& 0.0096& 0.0149&  0.0236 \\
  %  caser\_onlynew &0.2643& 0.3505& 0.4229 &  0.1810& 0.2089& 0.2274  \\
    caser\_fine-tuning &0.2658& 0.3516& 0.4259& 0.1817&   0.2096& 0.2285 \\
    Transfer & 0.2815& 0.3794& 0.4498 & 0.1838&0.2156&0.2336 \\
    %Transfer &0.2734& 0.3595 &0.4273&  0.1873&0.2152& 0.2325  \\
    %transfer-2 & 0.2769 & 0.3707& 0.4446 & 0.1752&0.2057&0.2245\\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}
  \caption{result of yelp}
  \label{tab:yelp-reslut}
  \begin{tabular}{ccccccl}
    \toprule
    methods &Recall@5 & Recall@10&Recall@20 & NDCG@5&NDCG@10&NDCG@20\\
    \midrule
    MF-full-retraining & 0.1764& 0.2822& 0.4118 & 0.1117& 0.1457& 0.1784\\
    MF-fine-tuning &0.1641& 0.2464& 0.3473&  0.1075& 0.1340&  0.1594  \\
    SPMF\_(7k-15w pool) & 0.1725& 0.2580& 0.3635 & 0.1136 & 0.1411 &0.1677 \\
    GRU4Rec & 0.1706& 0.2764&  0.4158& 0.1080&      0.1420&      0.1771\\
    %GRU4Rec-onlynew &0.1109& 0.1928 &0.3139 & 0.0683 &0.0946& 0.1250\\
    %caser-add &0.2143& 0.3263& 0.4648& 0.1404& 0.1764& 0.2114 \\
    caser\_fine-tuning &0.2195& 0.3320& 0.4565& 0.1440 & 0.1802 & 0.2117 \\
    Transfer &0.2225&0.3353&0.4720&0.1463&    0.1826 & 0.2171 \\  
    \bottomrule
  \end{tabular}
\end{table*}


\begin{table*}
\caption{news ablation studies}
\label{tab:cnn-mlp-news}
\begin{tabular}{ccccccl}
\toprule
method & recall@5 & recall@10 & recall@20       & ndcg@5 & ndcg@10 & ndcg@20 \\ 
\midrule
MLP & 0.1740 & 0.2479 & 0.3297&0.1146&0.1385&0.1591\\
CNN & 0.2815& 0.3794& 0.4498 & 0.1838&0.2156&0.2336 \\
CNN\_stop  & 0.2536&0.3618&0.4301&0.1611&0.1963&0.2173 \\
CNN\_nofuture & 0.2103&0.3294&0.4270&0.1293&0.1678&0.1927\\

%CNN &0.2225&0.3353&0.4720&0.1463&    0.1826 & 0.2171 \\
%CNN & 0.2769 & 0.3707& 0.4446 & 0.1752&0.2057&0.2245\\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}
\caption{yelp ablation studies}
\label{tab:cnn-mlp}
\begin{tabular}{ccccccl}
\toprule
method & recall@5 & recall@10 & recall@20       & ndcg@5 & ndcg@10 & ndcg@20 \\ 
\midrule
MLP&0.2166 & 0.3281& 0.4672&0.1427& 0.1786& 0.2137\\
%MLP  & 0.2109& 0.3218 & 0.4618 & 0.1386 & 0.1743  & 0.2096  \\
CNN &0.2225&0.3353&0.4720&0.1463&    0.1826 & 0.2171 \\
%CNN\_stop(no optimize when testing) & 0.1732& 0.2724& 0.4030& 0.1121& 0.1439& 0.1769\\
CNN\_stop & 0.2020& 0.3047& 0.4309&0.1352 &  0.1697&  0.1973\\
cnn\_nofuture& 0.1444& 0.2271& 0.3294& 0.0921&  0.1187& 0.1445\\
\bottomrule
\end{tabular}
\end{table*}








 
